On Robust Tie-line Scheduling in Multi-Area Power Systems

The tie-line scheduling problem in a multi-area power system seeks to optimize tie-line power flows across areas that are independently operated by different system operators (SOs). In this paper, we leverage the theory of multi-parametric linear programming to propose algorithms for optimal tie-line scheduling within a deterministic and a robust optimization framework. Through a coordinator, the proposed algorithms are proved to converge to the optimal schedule within a finite number of iterations. A key feature of the proposed algorithms, besides their finite step convergence, is the privacy of the information exchanges; the SO in an area does not need to reveal its dispatch cost structure, network constraints, or the nature of the uncertainty set to the coordinator. The performance of the algorithms is evaluated using several power system examples.

==> Application.tex <==
%application methods \subsection{System partition}
\indent Fluctuations of power flow distribution can be attributed as fluctuation of power injections. Hence in this paper, fluctuation sources are modeled as injections. For fluctuation source $i$, we know its connecting node $k_{i}$, standard error for fluctuation of active and reactive power injections $\Delta P_{i}$ and $\Delta Q_{i}$. The values for $\Delta P_{i}$ and $\Delta Q_{i}$ can be assigned by operation experience. Especially, for wind farms, these values can be set according to the variance of real-time wind power prediction. Subsequently, the fluctuation level of power flow on branch $l$, denoted by $\Delta P_{l}$ and $\Delta Q_{l}$, can be computed by:
\begin{equation}
\begin{array}{lll}
\Delta P_{l}&=&\sum \limits_{i=1}^{n}|S_{P}(k_{i},l)\Delta P_{i}|,\\
\Delta Q_{l}&=&\sum \limits_{i=1}^{n}|S_{Q}(k_{i},l)\Delta Q_{i}|.
\end{array}\label{eq:line_delta}
\end{equation}
where $S_{P}(k_{i},l)$ is the entry corresponding to node $k_{i}$ and branch $l$ in active power shift factor matrix, and $S_{Q}(k_{i},l)$ is the same entry in reactive power shift factor matrix. Scalar $n$ denotes the number of fluctuation sources.\\
\indent The fluctuation level of node $j$ is $\Delta_{j}$ defined by:
\begin{equation}
\begin{array}{lll}
\Delta P_{j}&=&\max \limits_{l\in \mathcal{A}_{j}}P_{l},\\
\Delta Q_{j}&=&\max \limits_{l\in \mathcal{A}_{j}}Q_{l},\\
\Delta_{j}&=&\sqrt{\Delta P_{j}^{2}+\Delta Q_{j}^{2}}.
\end{array}\label{eq:node_delta}
\end{equation}
where $\mathcal{A}_{j}$ denotes the adjacent branch set for node $j$.\\
\indent With the fluctuation level of each node, the system node set $\mathcal{N}$ is partitioned into steady area node set $\mathcal{N_{S}}$, quasi-steady area node set $\mathcal{N_{Q}}$ and fluctuant area node set $\mathcal{N_{F}}$:
\begin{equation}
\begin{array}{lll}
\mathcal{N_{S}}&=&\{j\in\mathcal{N}|\Delta_{j}\leq\epsilon_{q}\},\\
\mathcal{N_{Q}}&=&\{j\in\mathcal{N}|\epsilon_{q}<\Delta_{j}\leq\epsilon_{f}\},\\
\mathcal{N_{F}}&=&\{j\in\mathcal{N}|\Delta_{j}>\epsilon_{f}\}.
\end{array}\label{eq:sys_partition}
\end{equation}
where $\epsilon_{q}$ and $\epsilon_{f}$ are artificial thresholds.\\
\indent Similarly, the system measurement set $\mathcal{M}$ is also partitioned into steady area measurement set $\mathcal{M_{S}}$, quasi-steady area measurement set $\mathcal{M_{Q}}$ and fluctuant area measurement set $\mathcal{M_{F}}$. The steady area measurement set $\mathcal{M_{S}}$ includes measurements for node in $\mathcal{N_{S}}$ and measurements for head (tail) side for branches whose head (tail) nodes are in $\mathcal{N_{S}}$.\\
\indent Note that the system partition can change with system operations. Hence it is necessary to update the system partition after system operations are scheduled.
\subsection{State estimation method}
\indent Take steady area as example, its states are denoted by vector $x_{S}$, and the states for nodes outside but adjacent to steady area are denoted by $x_{BS}$. Then the measurement functions for steady area are:
\begin{equation}
z_{S}=h_{S}(x_{S},x_{BS})+e_{S}.\label{eq:meas_steadyarea}
\end{equation}
where $z_{S}$, $h_{S}$ and $e_{S}$ denote, respectively, measurement values, measurement functions and errors for measurement set $\mathcal{M_{S}}$.\\
\indent The state estimates for steady area are obtained by solving following weighted least square problem:
\begin{equation}
\begin{array}{ll}
\min \limits_{x_{S}}& (z_{S}-h_{S}(x_{S},x_{BS}))^{\dagger}W_{S}(z_{S}-h_{S}(x_{S},x_{BS})).
\end{array}\label{eq:semodel_steadyarea}
\end{equation}
where $W_{S}$ is the weight matrix for measurement set $\mathcal{M_{S}}$.
\indent Model (\ref{eq:semodel_steadyarea}) estimates the states in steady area with states in quasi-steady and fluctuant areas fixed. Similarly, the state estimation in quasi-steady and fluctuant areas will only update their own states as well. At any time moment $t$, the state estimates for the entire power system is given by:
\begin{equation}
\hat{x}=[\hat{x}_{S},\hat{x}_{Q},\hat{x}_{F}].\label{eq:se_fusion}
\end{equation}
where $\hat{x}_{S}$, $\hat{x}_{Q}$ and $\hat{x}_{F}$ are newest state estimates for steady area, quasi-steady area and fluctuant area, respectively.
\indent There are several effective hybrid PSSE methods, in this paper we use the method in \cite{Zhou_PWRS2006} for hybrid PSSE. The PSSE method with pure PMU measurements are given in section \ref{sec:concept}. 
